Nonlinear Diffusion Acceleration of the Least-Squares Transport Equation in Geometries with Voids

In this paper we show the extension of the Nonlinear-Diffusion Acceleration (NDA) to geometries containing small voids using a weighted least-squares (WLS) high order equation. Even though the WLS equation is well defined in voids, the low-order drift diffusion equation was not defined in materials with a zero cross section. This paper derives the necessary modifications to the NDA algorithm. We show that a small change to the NDA closure term and a non-local definition of the diffusion coefficient solve the problems for voids regions. These changes do not affect the algorithm for optical thick material regions, while making the algorithm well defined in optically thin ones. We use a Fourier analysis to perform an iterative analysis to confirm that the modifications result in a stable and efficient algorithm. Numerical results of our method will be presented in the second part of the paper. We test this formulation with a small, one-dimensional test problem. Additionally we present results for a modified version of the C5G7 benchmark containing voids as a more complex, reactor like problem. We compared our results to PDT, Texas A\&M's transport code, utilizing a first order discontinuous formulation as reference and the self-adjoint angular flux equation with void treatment (SAAFt), a different second order form. The results indicate, that the NDA WLS performed comparably or slightly worse then the asymmetric SAAFt, while maintaining a symmetric discretization matrix.

==> common/macros.tex <==
\makeatletter
% prevent a package from loading
\newcommand{\dontusepackage}[2][]{%
    \@namedef{ver@#2.sty}{9999/12/31}%
    \@namedef{opt@#2.sty}{#1}
}

% a macro to load packages only if they are not yet loaded, needed for combination of beamer and hyperref
\newcommand{\usepackagesave}[2][{}]{
    \ltx@ifpackageloaded{#2}{}{
        \usepackage[#1]{#2}}
}

% prevent packages from loading depending on document class

% standalone
\@ifclassloaded{standalone}%
{
    \dontusepackage{geometry}
}
{}%

\makeatother


==> content/acknowledgements.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%  New template code for TAMU Theses and Dissertations starting Fall 2016.
%
%  Author: Sean Zachary Roberson
%	 Version 3.16.09
%  Last updated 9/12/2016
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                           ACKNOWLEDGMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Acknowledgments}
This material is based upon work supported by the Department of Energy, Battelle Energy Alliance, LLC, under Award Number DE-AC07-05ID14517.
